Motion Planning via Manifold Samples

We present a general and modular algorithmic framework for path planning of robots. Our framework combines geometric methods for exact and complete analysis of low-dimensional configuration spaces, together with practical, considerably simpler sampling-based approaches that are appropriate for higher dimensions. In order to facilitate the transfer of advanced geometric algorithms into practical use, we suggest taking samples that are entire low-dimensional manifolds of the configuration space that capture the connectivity of the configuration space much better than isolated point samples. Geometric algorithms for analysis of low-dimensional manifolds then provide powerful primitive operations. The modular design of the framework enables independent optimization of each modular component. Indeed, we have developed, implemented and optimized a primitive operation for complete and exact combinatorial analysis of a certain set of manifolds, using arrangements of curves of rational functions and concepts of generic programming. This in turn enabled us to implement our framework for the concrete case of a polygonal robot translating and rotating amidst polygonal obstacles. We demonstrate that the integration of several carefully engineered components leads to significant speedup over the popular PRM sampling-based algorithm, which represents the more simplistic approach that is prevalent in practice. We foresee possible extensions of our framework to solving high-dimensional problems beyond motion planning.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Sampling based methods stemmed from the Probablistic 
Motion Planner (PRM)~\cite{Kavraki-PRM} which is a 
simple yet powerful multi-query planner. In order to 
overcome the so-called tight passage problem, several 
variants have been proposed 
including~\cite{Bridge-test},~\cite{Gaussion-sampling} 
and more. Combinatorial based motion planning techniques 
include Minkowski sums for translating robots \cite{CG-alg-app}, 
applying arrangements to the critical curves of a 
problem \commentBegin TBD \commentEnd and more.

Several works attempt to hybridize the exact complete 
solutions offered by combinatorial based methods for 
low dimensional configuration spaces with the simple 
and efficient solutions offered by sampling based methods. 
De Berg et al.\cite{CG-alg-app} suggest a general 
method where $\calC$ is sliced into layers of fixed 
rotation. Each layer is computed by a complete planner 
for 2D translational robot using cell decomposition. 
Two slices are connected if the subdivisions from both 
slices overlap. 

Implementations based on the method described include 
the following works: Halperin et al.~\cite{hybrid-disks} 
suggested a hybridized scheme for coordinating two 
disk robots. Zhang et al. \cite{hybrid-cell-decomp} 
combine approximate cell decomposition with PRMs and 
Ming-Lien~\cite{hybrid-mink} suggests a hybrid 
planner by dividing the configuration space to 
translational and rotational components acheiving high results 

\commentBegin State shortcoming of works \commentEnd
%limited the movement to either purely rotational or purely translational sections.
\commentBegin Work on translating and rotating robots \commentEnd
%\subsection{Sampling based methods}
%\commentBegin Should be around 0.3 pages \commentEnd
%Sampling Based Motion Planning attempt to capture the connectivity of the free space by sampling the configuration space, hence avoiding an explicit representation of the configuration space. Sampling based approaches may be divided into two multi-query planners (PRM) and single query planners (RRT,EST)\cite{Kavraki-PRM-I}. 
%
%\commentBegin Should PRM demonstration be included? \commentEnd
%A PRM - type algorithm usually consists of two stages: A sampling stage and a query stage. 
%
%In the sampling stage, the configuration space is sampled to produce collision free configurations. An attempt to connect close configurations is done via a \emph{local planner}. The \emph{local planner} typically uses dense sampling between the configurations in order to determine if a collision free path exists. This yields a graph in the configuration space where the vertices are the free configurations sampled and the edges are the local paths.
%
%In the query stage the source and target configurations are added to the graph and connected to nearby configurations using the local planner, then, the graph is searched for a path between the nodes to yield a free path in the configuration space.
%
%Probabilistic sampling-based methods for motion planning were shown to be particularly useful when the configuration space is high dimensional but fails (in terms of running time) when tackeled with the so-called ''narrow passage'' problem.

%
%\subsection{Combinatorial based methods}
%\commentBegin Should be around 0.3 pages \commentEnd
%Combinatorial motion planning approaches find paths through the continuous configuration space without resorting to approximations. Some of the methods are impractical for high dimensional configuration spaces but for one of the simplest, most fundamental of motion planning problems, namely a polygonal robot translating in a room amidst polygonal obstacles, an exact and efficient combinatorial motion planning algorithm exists using \emph{minkowski sums}
%
%\subsubsection{Minkowski Sums}
%
%Given two sets $P,Q \in R^d$, their Minkowski sum, denoted as $P \oplus Q$, is their point-wise sum, namely the set: $P \oplus Q = \{p + q | p\in P, q\in Q\} $. Minkowski sums can be used to detect collision between and compute relative placement of two sets. Let $-Q$ denote the reflection of $Q$ about the origin. As $p \in Q$, then $-p \in -Q$ and thus $ P \oplus (-Q)$ contains the origin as $(0, 0) = p + (-p)$. The reverse direction is also true: if $(0, 0) \in P \oplus (-Q)$, then $P \cap Q \neq \emptyset$. Thus, the sum $ P \oplus -Q$  is the configuration-space induced by the obstacle $P$ with respect to a translating robot $Q$. 
%
%These properties of Minkowski sums lead to immediate applications in combinatorial motion planning for a translating polygonal robot:
%\begin{itemize}
%	\item {\bf Collision detection}: Detecting collision between a robot $R$ and an obstacle $O$ can be done by testing if the origin $o$ lies inside the Minkowski sum of the reflected robot and the obstacle $ M = -R \oplus O$ . 
%	\item {\bf Computing the Configuration space}: Let $P_1, \ldots P_m$ be the set of polygonal obstacles and let $r_0 \in R$ be a reference point on the robot $R$. Translating $R$ such that $r_0$ coincides with the origin, and reflecting the robot about the origin leads us to $-R$. Thus $\Cforb = \bigcup^{i=1}_{m} O_i \oplus -R$
%	\item {\bf Determening if a collision-free path exists}: given a start location $s$ and a target location $t$, we whish to determine whether there exists a collision-free path connecting $s$ and $t$. We simply compute $\Cforb$, and consider its complement, $\Cfree = \R^2 \setminus \Cforb$. A path exists between $s$ and $t$ iff these two points lie in the same connected component of $\Cfree$. 
%\end{itemize}
%
%As the cells of the configuration space may be complicated a vertical decomposition is usually applied to the configuration space in order to subdivide it into simple cells with bounded complexity where a path is found. 
%
%Figure \ref{fig:workspace} demonstrates a workspace consisting of polygonal obstacles (shaded in blue) and a disk robot (shaded in green), while figure \ref{fig:Configuration-Space} illustrates the corresponding Configuration Space computed using the minkowski sum of the reflected robot and the obstacles. figure \ref{fig:path-in-fs} demonstrates a decomposition of the free space computed using minkowski sums into cells and a path planned in the decomposed free space
%
%\begin{figure}[htbp]
%\begin{minipage}{0.33\linewidth}
%\centering
%\includegraphics[width=0.9\linewidth,clip]{C:/Users/Salzmans/Documents/Oren/Studies/Thesis/workspace_example1.jpg}
%\caption{Workspace of a disc}
%\label{fig:workspace}
%\end{minipage}%
%\begin{minipage}{0.33\linewidth}
%\centering
%\includegraphics[width=0.9\linewidth,clip]{C:/Users/Salzmans/Documents/Oren/Studies/Thesis/configuration_space_example1.jpg}
%\caption{Configuration Space}
%\label{fig:Configuration-Space}
%\end{minipage}
%\begin{minipage}{0.33\linewidth}
%\centering
%\includegraphics[width=0.9\linewidth,clip]{C:/Users/Salzmans/Documents/Oren/Studies/Thesis/path_in_dec_free_space.jpg}
%\caption{Path in decomposed free space}
%\label{fig:path-in-fs}
%\end{minipage}
%\end{figure}

